Towards Radar Emitter Recognition in Changing Environments with Domain Generalization

Analyzing radar signals from complex Electronic Warfare (EW) environment is a non-trivial task.However, in the real world, the changing EW environment results in inconsistent signal distribution, such as the pulse repetition interval (PRI) mismatch between different detected scenes.In this paper, we propose a novel domain generalization framework to improve the adaptability of signal recognition in changing environments.Specifically, we first design several noise generators to simulate varied scenes. Different from conventional augmentation methods, our introduced generators carefully enhance the diversity of the detected signals and meanwhile maintain the semantic features of the signals. Moreover, we propose a signal scene domain classifier that works in the manner of adversarial learning. The proposed classifier guarantees the signal predictor to generalize to different scenes. Extensive comparative experiments prove the proposed method's superiority.

==> draft.tex <==
The method can recognize PRI modulation as long as the data volume is large enough and the PRI patterns are simple. However, the methods require a lot of manpower and time when modeling and statistics, and it is difficult to recognize emitter accurately.

\item we create a standard data set for real world radar emitter recognition.



\begin{figure*}
\centering
\subfigure[]{
\includegraphics[scale=0.5]{rst_a.png}
}
\hspace{0.5in}
\subfigure[]{
\includegraphics[scale=0.5]{rst_b.png}
}
\caption{The recognition accuracy of our method for (a) emitters with different PRI modulations (b) emitters with STG PRI but different parameters in different error environment.}
\label{fig:results}
%
\end{figure*}





\begin{table*}[ht]
\centering
\setlength{\tabcolsep}{8mm}{
\begin{tabular}{lllllll}
\hline
Methods     & CST     & JIT     & SLD     & WOB     & D\&S     &avg.STG \\
\hline
CNN \cite{2018LiCNN}        & 35.0      & 30.0      & 57.0      & 60.0  &51.0   &49.2      \\
A-RNN \cite{2020LiRNN}      & 40.0      & 40.0      & 59.0      & 57.0  &53.0   &50.6      \\
ACSE \cite{2020ACSE}       & 40.0      & 38.0      & 53.0      & 58.0  &54.0   &48.8      \\
TCN \cite{2021TCN}        & 46.0      & 48.0      & 56.0      & 54.0  &58.0   &51.4       \\
ERM \cite{ERM}        & 49.0      & 54.0      & 62.0      & 64.0  &59.0   &56.6      \\
d-SNE \cite{2019d-SNE}      & 58.0      & 56.0      & 64.0      & 62.0  &59.0   &59.0      \\
MADA \cite{2020MADA}       & 56.0      & 55.0      & 65.0      & 70.0  &62.0   &60.6      \\
SG-DANN     & {\bf67.0} & {\bf59.0} & {\bf78.0} & {\bf85.0} &{\bf81.0}   &{\bf70.6}      \\

\hline
\end{tabular}
}
\caption{Recognition accuracy of radar emitter with different PRI modulation.}
\label{tab:tab2}
\end{table*}


\begin{table*}[ht]
\centering
\setlength{\tabcolsep}{9mm}{
\begin{tabular}{llllll}
\hline
Methods     & STG1     & STG2     & STG3     & STG4     & STG5  \\
\hline
CNN \cite{2018LiCNN}        & 51.0      & 56.0      & 47.0      & 43.0  &49.0      \\
A-RNN \cite{2020LiRNN}      & 52.0      & 51.0      & 45.0      & 49.0  &56.0      \\
ACSE \cite{2020ACSE}       & 50.0      & 53.0      & 49.0      & 47.0  &45.0      \\
TCN \cite{2021TCN}        & 56.0      & 53.0      & 47.0      & 47.0  &54.0      \\
ERM \cite{ERM}        & 62.0      & 51.0      & 51.0      & 56.0  &63.0      \\
d-SNE \cite{2019d-SNE}      & 63.0      & 61.0      & 53.0      & 56.0  &62.0      \\
MADA \cite{2020MADA}       & 62.0      & 60.0      & {\bf61.0} & 57.0  &63.0      \\
SG-DANN     & {\bf76.0} & {\bf74.0} & {\bf61.0} & {\bf69.0} &{\bf73.0}     \\

\hline
\end{tabular}
}
\caption{Recognition accuracy of radar emitter with STG PRI but different parameters.}
\label{tab:tab3}
\end{table*}

\cite{1999GPNoone} firstly applied multilayer perception (MLP) to PRI modulation recognition, which made a breakthrough in radar recognition accuracy but needed to input extracted high dimensional features to MLP.
\cite{2010Hierarchical} utilized a two-stage hierarchical classification scheme and extracted subpatterns to seek for features of PRI sequences to identify the PRI modulation, but the model broke down when high ratios of noise were added.



We compare our method with the following methods. (1) Convolutional Neural Network (CNN)\cite{2018LiCNN}is the baseline method trained with only the cross-entropy loss. (2) Attention-Based Recurrent Neural Networks (A-RNN)\cite{2020LiRNN} extends words embedding technique by converting PRI into discrete tokens using preset units. (3)Asymmetric Convolution Squeeze-and-Excitation network (ACSE)\cite{2020ACSE} uses the normalized autocorrelation features as input. (4)temporal convolutional network (TCN)\cite{2021TCN} uses 30-dim features as input. (5) Empirical Risk Minimization (ERM)\cite{ERM} is the DG baseline method trained with the cross-entropy loss. (6) Domain adaptation using stochastic neighborhood embedding (d-SNE)\cite{2019d-SNE} minimizes the maximum distance between sample pairs of the same class and maximizes the minimum distance among sample pairs of different classes. (7) Meta-Learning based Adversarial Domain Augmentation (MADA)\cite{2020MADA} minimizes the distance of semantic space and maximize the distance of PRI value space to generate more effective samples.

We train the models with 90\% signal PRI sequences in the train set, validate the models on the rest of the train set, and evaluate the model on the test sets with different error environments.We calculate the mean accuracy on each set as the evaluation index. 



{\bf constant PRI:} A constant PRI sequence always has a fixed value. It can be formulated as: $PRI_i = c$, where $c$ is a constant.

{\bf jittered PRI:} The values of jittered PRI sequences jittered around a certain constant value. It can be formulated as: $PRI_i = c + \delta$, where $\delta$ is usually a Gaussian variable with variance less than 30\% of the mean PRI.

{\bf sliding PRI:} A sliding PRI has a periodic monotonic increase or decrease.It can be formulated as: $PRI_i = c + k*mod(i, M)$, where $k$ is the sliding slope and $M$ is the sliding period.

{\bf wobulated PRI:} The values of wobulated PRI sequence usually vary according to a sinusoidal function. It can be formulated as: $PRI_i = c + A \sin(\omega i + \varphi)$, where $A$ is the modulation amplitude, $\omega$ is the frequency, $\varphi$ is the phase .

{\bf staggered PRI:} There are M fixed values appear cyclically in order in a stagger PRI sequence.It can be formulated as: $PRI_i = y_n$, where each $y_n$ is a pre-defined value and $n = mod(i,M)$.

{\bf dwell and switch PRI:} Like the staggered PRI, there are several stable values in the D\&S PRI sequence, but each value may be repeated for some period.


4.3
The existing radar emitter recognition methods did not consider the potential mismatch between the training and the testing samples. Thus it is meaningless to add unlabeled test data for training.
